The relationship between variable and polarized optical spectral components of luminous type 1 non-blazar quasars

Optical spectropolarimetry carried out by Kishimoto et al. (2004) has shown that several luminous type 1 quasars show a strong decrease of the polarized continuum flux in the rest-frame near-UV wavelengths of $\lambda<4000$\AA. In the literature, this spectral feature is interpreted as evidence of the broadened hydrogen Balmer absorption edge imprinted in the accretion disk thermal emission due to the disk atmospheric opacity effect. On the other hand, the quasar flux variability studies have shown that the variable continuum component in UV-optical spectra of quasars, which is considered to be a good indicator of the intrinsic spectral shape of the accretion disk emission, generally have significantly flat spectral shape throughout the near-UV to optical spectral range. To examine whether the disk continuum spectral shapes revealed as the polarized flux and as the variable component spectra are consistent with each other, we carry out multi-band photometric monitoring observations for a sample of four polarization-decreasing quasars of Kishimoto et al. (2004) (4C09.72, 3C323.1, Ton 202, and B2 1208+32) to derive the variable component spectra and compare the spectral shape of them with that of the polarized flux spectra. Contrary to expectation, we confirm that the two spectral components of these quasars have totally different spectral shape in that the variable component spectra are significantly bluer compared to the polarized flux spectra. This discrepancy in the spectral shape may imply either (1) the decrease of polarization degree in the rest-frame UV wavelengths is not indicating the Balmer absorption edge feature but is induced by some unknown (de)polarization mechanisms, or (2) the UV-optical flux variability is occurring preferentially at the hot inner radii of the accretion disk and thus the variable component spectra do not reflect the whole accretion disk emission.

==> table2.tex <==



\begin{table} 
\tbl{KWFC $u$, $g$, $r$, $i$, and $z$-band light curves for B2~1208+32, Ton~202, 3C323.1, and 4C09.72.}{%
\begin{tabular}{lcccc}  
\hline\noalign{\vskip3pt} 
\multicolumn{1}{c}{Name} & MJD & Magnitude & Error in magnitude & Band \\  [2pt] 
\hline\noalign{\vskip3pt} 
B2~1208+32 & 57164.47822 & 16.9528 & 0.0306 &  $u$\\
B2~1208+32 & 57390.64625 & 17.1045 & 0.0167 &  $u$\\
B2~1208+32 & 57402.62973 & 17.0845 & 0.0170 &  $u$\\
B2~1208+32 & 57407.78441 & 17.1105 & 0.0258 &  $u$\\
B2~1208+32 & 57419.86152 & 17.0244 & 0.0291 &  $u$\\
B2~1208+32 & 57420.58574 & 17.0492 & 0.0155 &  $u$\\
B2~1208+32 & 57433.54302 & 17.0783 & 0.0285 &  $u$\\
B2~1208+32 & 57445.67669 & 17.0510 & 0.0259 &  $u$\\
B2~1208+32 & 57446.51312 & 17.0809 & 0.0336 &  $u$\\
B2~1208+32 & 57129.59170 & 16.8277 & 0.0081 &  $g$\\
B2~1208+32 & 57151.61124 & 16.8178 & 0.0109 &  $g$\\
B2~1208+32 & 57152.61655 & 16.8332 & 0.0088 &  $g$\\
B2~1208+32 & 57161.49397 & 16.8084 & 0.0092 &  $g$\\
B2~1208+32 & 57164.45771 & 16.8235 & 0.0154 &  $g$\\
B2~1208+32 & 57171.56550 & 16.8284 & 0.0144 &  $g$\\
B2~1208+32 & 57188.53751 & 16.8669 & 0.0773 &  $g$\\
B2~1208+32 & 57390.62650 & 16.9786 & 0.0078 &  $g$\\
B2~1208+32 & 57402.61074 & 16.9643 & 0.0075 &  $g$\\
B2~1208+32 & 57407.76236 & 16.9652 & 0.0154 &  $g$\\
B2~1208+32 & 57419.84006 & 16.9625 & 0.0092 &  $g$\\
B2~1208+32 & 57420.56788 & 16.9750 & 0.0069 &  $g$\\
B2~1208+32 & 57433.52307 & 17.0106 & 0.0135 &  $g$\\
B2~1208+32 & 57445.65384 & 16.9384 & 0.0154 &  $g$\\
B2~1208+32 & 57446.49379 & 17.0004 & 0.0136 &  $g$\\
B2~1208+32 & 57129.60164 & 16.8564 & 0.0082 &  $r$\\
B2~1208+32 & 57147.56783 & 16.8481 & 0.0196 &  $r$\\
B2~1208+32 & 57151.62401 & 16.8520 & 0.0114 &  $r$\\
B2~1208+32 & 57152.62555 & 16.8404 & 0.0097 &  $r$\\
B2~1208+32 & 57164.47184 & 16.8248 & 0.0117 &  $r$\\
B2~1208+32 & 57169.51788 & 16.8488 & 0.0222 &  $r$\\
B2~1208+32 & 57171.57981 & 16.8679 & 0.0182 &  $r$\\
B2~1208+32 & 57390.63837 & 16.9526 & 0.0072 &  $r$\\
B2~1208+32 & 57402.62246 & 16.9599 & 0.0066 &  $r$\\
B2~1208+32 & 57407.77540 & 16.9495 & 0.0165 &  $r$\\
B2~1208+32 & 57419.85302 & 16.9583 & 0.0102 &  $r$\\
B2~1208+32 & 57420.57850 & 16.9519 & 0.0065 &  $r$\\
B2~1208+32 & 57433.53479 & 16.9322 & 0.0109 &  $r$\\
B2~1208+32 & 57445.66866 & 16.9745 & 0.0146 &  $r$\\
B2~1208+32 & 57446.50554 & 16.9519 & 0.0119 &  $r$\\
B2~1208+32 & 57129.59667 & 16.8495 & 0.0117 &  $i$\\
B2~1208+32 & 57147.56294 & 16.8380 & 0.0225 &  $i$\\
B2~1208+32 & 57151.61952 & 16.8633 & 0.0210 &  $i$\\
B2~1208+32 & 57152.62102 & 16.8415 & 0.0146 &  $i$\\
B2~1208+32 & 57161.50834 & 16.8420 & 0.0191 &  $i$\\
B2~1208+32 & 57164.46611 & 16.8427 & 0.0131 &  $i$\\
B2~1208+32 & 57169.49165 & 16.8410 & 0.0242 &  $i$\\
B2~1208+32 & 57171.57263 & 16.8454 & 0.0171 &  $i$\\
B2~1208+32 & 57201.47058 & 16.8520 & 0.0202 &  $i$\\
B2~1208+32 & 57390.63227 & 16.9447 & 0.0110 &  $i$\\
B2~1208+32 & 57402.61663 & 16.9356 & 0.0095 &  $i$\\
B2~1208+32 & 57407.76882 & 16.9310 & 0.0152 &  $i$\\
B2~1208+32 & 57419.84683 & 16.9394 & 0.0134 &  $i$\\
B2~1208+32 & 57420.56973 & 16.9364 & 0.0088 &  $i$\\
B2~1208+32 & 57433.52894 & 16.9126 & 0.0119 &  $i$\\
B2~1208+32 & 57445.66211 & 16.9229 & 0.0159 &  $i$\\
B2~1208+32 & 57446.49971 & 16.9238 & 0.0168 &  $i$\\
B2~1208+32 & 57129.61147 & 16.2518 & 0.0131 &  $z$\\
B2~1208+32 & 57147.57756 & 16.2554 & 0.0198 &  $z$\\
B2~1208+32 & 57151.63301 & 16.2908 & 0.0175 &  $z$\\
B2~1208+32 & 57152.63453 & 16.2675 & 0.0208 &  $z$\\
B2~1208+32 & 57164.48647 & 16.3289 & 0.0152 &  $z$\\
B2~1208+32 & 57169.56646 & 16.2486 & 0.0246 &  $z$\\
B2~1208+32 & 57390.65486 & 16.3632 & 0.0095 &  $z$\\
B2~1208+32 & 57402.63836 & 16.3344 & 0.0079 &  $z$\\
B2~1208+32 & 57407.79306 & 16.3286 & 0.0111 &  $z$\\
B2~1208+32 & 57419.86828 & 16.3120 & 0.0188 &  $z$\\
B2~1208+32 & 57420.59435 & 16.3075 & 0.0066 &  $z$\\
B2~1208+32 & 57433.55081 & 16.3229 & 0.0081 &  $z$\\
B2~1208+32 & 57445.68639 & 16.2809 & 0.0112 &  $z$\\
B2~1208+32 & 57446.52145 & 16.3229 & 0.0127 &  $z$\\
Ton~202 & 57129.63296 & 16.3382 & 0.0223 &  $u$\\
Ton~202 & 57151.65279 & 16.2994 & 0.0224 &  $u$\\
Ton~202 & 57152.65318 & 16.2922 & 0.0206 &  $u$\\
Ton~202 & 57169.57134 & 16.2974 & 0.0285 &  $u$\\
Ton~202 & 57185.69187 & 16.3394 & 0.0167 &  $u$\\
Ton~202 & 57229.50221 & 16.3552 & 0.0218 &  $u$\\
Ton~202 & 57390.74597 & 16.6332 & 0.0201 &  $u$\\
Ton~202 & 57402.73030 & 16.6139 & 0.0117 &  $u$\\
Ton~202 & 57407.82143 & 16.5937 & 0.0159 &  $u$\\
Ton~202 & 57420.68653 & 16.6168 & 0.0111 &  $u$\\
Ton~202 & 57433.64743 & 16.6060 & 0.0136 &  $u$\\
Ton~202 & 57445.71448 & 16.5885 & 0.0279 &  $u$\\
Ton~202 & 57129.61581 & 16.1975 & 0.0042 &  $g$\\
Ton~202 & 57151.63786 & 16.2224 & 0.0068 &  $g$\\
Ton~202 & 57152.63260 & 16.2174 & 0.0056 &  $g$\\
Ton~202 & 57162.75600 & 16.2525 & 0.0108 &  $g$\\
Ton~202 & 57166.52074 & 16.2105 & 0.0109 &  $g$\\
Ton~202 & 57169.52354 & 16.2049 & 0.0105 &  $g$\\
Ton~202 & 57185.67310 & 16.2644 & 0.0049 &  $g$\\
Ton~202 & 57229.48116 & 16.2891 & 0.0080 &  $g$\\
Ton~202 & 57390.72878 & 16.5235 & 0.0066 &  $g$\\
Ton~202 & 57402.71138 & 16.5328 & 0.0053 &  $g$\\
Ton~202 & 57407.80132 & 16.5512 & 0.0081 &  $g$\\
Ton~202 & 57420.66769 & 16.5717 & 0.0048 &  $g$\\
Ton~202 & 57433.62829 & 16.5723 & 0.0081 &  $g$\\
Ton~202 & 57445.69447 & 16.5563 & 0.0170 &  $g$\\
Ton~202 & 57129.62768 & 16.2148 & 0.0051 &  $r$\\
Ton~202 & 57143.66684 & 16.2382 & 0.0208 &  $r$\\
Ton~202 & 57151.64777 & 16.2359 & 0.0063 &  $r$\\
Ton~202 & 57152.64821 & 16.2232 & 0.0057 &  $r$\\
Ton~202 & 57169.53388 & 16.2304 & 0.0101 &  $r$\\
Ton~202 & 57185.68469 & 16.2657 & 0.0057 &  $r$\\
Ton~202 & 57229.49773 & 16.3006 & 0.0060 &  $r$\\
Ton~202 & 57390.74035 & 16.5077 & 0.0061 &  $r$\\
Ton~202 & 57402.72311 & 16.5142 & 0.0049 &  $r$\\
Ton~202 & 57407.81377 & 16.5188 & 0.0073 &  $r$\\
Ton~202 & 57420.67930 & 16.5297 & 0.0045 &  $r$\\
Ton~202 & 57433.64006 & 16.5287 & 0.0065 &  $r$\\
Ton~202 & 57445.70679 & 16.5174 & 0.0157 &  $r$\\
Ton~202 & 57129.62254 & 16.2732 & 0.0074 &  $i$\\
Ton~202 & 57143.66195 & 16.2470 & 0.0248 &  $i$\\
Ton~202 & 57151.64276 & 16.2699 & 0.0084 &  $i$\\
Ton~202 & 57152.64333 & 16.2830 & 0.0087 &  $i$\\
Ton~202 & 57162.75973 & 16.3021 & 0.0268 &  $i$\\
Ton~202 & 57169.52871 & 16.3066 & 0.0125 &  $i$\\
Ton~202 & 57185.67889 & 16.3140 & 0.0074 &  $i$\\
Ton~202 & 57229.49224 & 16.3416 & 0.0062 &  $i$\\
Ton~202 & 57390.73455 & 16.5105 & 0.0086 &  $i$\\
Ton~202 & 57402.71724 & 16.5250 & 0.0075 &  $i$\\
Ton~202 & 57407.80757 & 16.5094 & 0.0101 &  $i$\\
Ton~202 & 57420.67348 & 16.5493 & 0.0064 &  $i$\\
Ton~202 & 57433.63421 & 16.5538 & 0.0085 &  $i$\\
Ton~202 & 57445.70058 & 16.5206 & 0.0171 &  $i$\\
Ton~202 & 57129.63807 & 15.7744 & 0.0098 &  $z$\\
Ton~202 & 57143.67660 & 15.8089 & 0.0226 &  $z$\\
Ton~202 & 57151.65777 & 15.7697 & 0.0093 &  $z$\\
Ton~202 & 57152.65819 & 15.7838 & 0.0114 &  $z$\\
Ton~202 & 57169.57657 & 15.7520 & 0.0123 &  $z$\\
Ton~202 & 57185.70015 & 15.8051 & 0.0107 &  $z$\\
Ton~202 & 57229.51437 & 15.8170 & 0.0068 &  $z$\\
Ton~202 & 57390.75660 & 15.9018 & 0.0072 &  $z$\\
Ton~202 & 57402.73898 & 15.9270 & 0.0065 &  $z$\\
Ton~202 & 57407.83050 & 15.9329 & 0.0080 &  $z$\\
Ton~202 & 57420.69511 & 15.9422 & 0.0058 &  $z$\\
Ton~202 & 57433.65610 & 15.9330 & 0.0071 &  $z$\\
Ton~202 & 57445.72362 & 15.8793 & 0.0117 &  $z$\\
3C323.1 & 57152.60449 & 16.3042 & 0.0215 &  $u$\\
3C323.1 & 57169.58268 & 16.3087 & 0.0288 &  $u$\\
3C323.1 & 57185.72664 & 16.3099 & 0.0117 &  $u$\\
3C323.1 & 57229.53120 & 16.1932 & 0.0091 &  $u$\\
3C323.1 & 57276.45946 & 16.1482 & 0.0108 &  $u$\\
3C323.1 & 57302.43283 & 16.1887 & 0.0135 &  $u$\\
3C323.1 & 57390.81315 & 16.1075 & 0.0109 &  $u$\\
3C323.1 & 57402.79654 & 16.0724 & 0.0089 &  $u$\\
3C323.1 & 57407.85700 & 16.0913 & 0.0118 &  $u$\\
3C323.1 & 57420.76717 & 16.0759 & 0.0090 &  $u$\\
3C323.1 & 57433.71224 & 16.0871 & 0.0085 &  $u$\\
3C323.1 & 57445.75129 & 16.0250 & 0.0290 &  $u$\\
3C323.1 & 57133.69661 & 16.3582 & 0.0053 &  $g$\\
3C323.1 & 57134.63122 & 16.3657 & 0.0060 &  $g$\\
3C323.1 & 57151.66308 & 16.3017 & 0.0081 &  $g$\\
3C323.1 & 57152.58978 & 16.3053 & 0.0056 &  $g$\\
3C323.1 & 57158.76580 & 16.2978 & 0.0151 &  $g$\\
3C323.1 & 57168.63109 & 16.2919 & 0.0125 &  $g$\\
3C323.1 & 57169.53946 & 16.2926 & 0.0108 &  $g$\\
3C323.1 & 57185.70844 & 16.2787 & 0.0059 &  $g$\\
3C323.1 & 57229.47736 & 16.1705 & 0.0055 &  $g$\\
3C323.1 & 57276.44243 & 16.1038 & 0.0034 &  $g$\\
3C323.1 & 57301.42832 & 16.1530 & 0.0050 &  $g$\\
3C323.1 & 57302.40406 & 16.1613 & 0.0050 &  $g$\\
3C323.1 & 57390.79408 & 16.1230 & 0.0055 &  $g$\\
3C323.1 & 57402.77770 & 16.0548 & 0.0039 &  $g$\\
3C323.1 & 57407.83790 & 16.0661 & 0.0058 &  $g$\\
3C323.1 & 57420.73072 & 16.0577 & 0.0043 &  $g$\\
3C323.1 & 57433.69325 & 16.0546 & 0.0039 &  $g$\\
3C323.1 & 57445.73129 & 16.0548 & 0.0155 &  $g$\\
3C323.1 & 57133.70679 & 16.1937 & 0.0065 &  $r$\\
3C323.1 & 57134.67736 & 16.2175 & 0.0065 &  $r$\\
3C323.1 & 57143.69210 & 16.1814 & 0.0159 &  $r$\\
3C323.1 & 57151.67197 & 16.1525 & 0.0139 &  $r$\\
3C323.1 & 57152.59959 & 16.1546 & 0.0053 &  $r$\\
3C323.1 & 57158.77473 & 16.1563 & 0.0236 &  $r$\\
3C323.1 & 57168.64057 & 16.1362 & 0.0103 &  $r$\\
3C323.1 & 57169.54962 & 16.1332 & 0.0086 &  $r$\\
3C323.1 & 57185.71945 & 16.1078 & 0.0049 &  $r$\\
3C323.1 & 57229.52412 & 16.0602 & 0.0045 &  $r$\\
3C323.1 & 57276.45406 & 16.0052 & 0.0035 &  $r$\\
3C323.1 & 57293.44652 & 16.0220 & 0.0114 &  $r$\\
3C323.1 & 57301.44058 & 15.9401 & 0.0518 &  $r$\\
3C323.1 & 57302.41855 & 16.0222 & 0.0051 &  $r$\\
3C323.1 & 57390.80566 & 15.9751 & 0.0045 &  $r$\\
3C323.1 & 57402.78935 & 15.9582 & 0.0034 &  $r$\\
3C323.1 & 57407.84958 & 15.9545 & 0.0050 &  $r$\\
3C323.1 & 57420.75988 & 15.9485 & 0.0036 &  $r$\\
3C323.1 & 57433.70500 & 15.9589 & 0.0035 &  $r$\\
3C323.1 & 57445.74304 & 15.9353 & 0.0132 &  $r$\\
3C323.1 & 57133.70170 & 16.1195 & 0.0069 &  $i$\\
3C323.1 & 57134.63607 & 16.1167 & 0.0069 &  $i$\\
3C323.1 & 57143.68701 & 16.0967 & 0.0170 &  $i$\\
3C323.1 & 57151.66822 & 16.0832 & 0.0085 &  $i$\\
3C323.1 & 57152.59467 & 16.0940 & 0.0078 &  $i$\\
3C323.1 & 57158.77029 & 16.1091 & 0.0214 &  $i$\\
3C323.1 & 57168.63661 & 16.0856 & 0.0095 &  $i$\\
3C323.1 & 57169.54450 & 16.0782 & 0.0102 &  $i$\\
3C323.1 & 57185.71343 & 16.0460 & 0.0070 &  $i$\\
3C323.1 & 57229.50736 & 16.0200 & 0.0058 &  $i$\\
3C323.1 & 57301.43415 & 15.9609 & 0.0060 &  $i$\\
3C323.1 & 57302.41151 & 15.9579 & 0.0074 &  $i$\\
3C323.1 & 57390.80047 & 15.9405 & 0.0073 &  $i$\\
3C323.1 & 57402.78350 & 15.9204 & 0.0049 &  $i$\\
3C323.1 & 57407.84370 & 15.8987 & 0.0070 &  $i$\\
3C323.1 & 57433.69916 & 15.9425 & 0.0073 &  $i$\\
3C323.1 & 57445.73719 & 15.9116 & 0.0126 &  $i$\\
3C323.1 & 57134.64100 & 15.5073 & 0.0082 &  $z$\\
3C323.1 & 57143.70212 & 15.5194 & 0.0135 &  $z$\\
3C323.1 & 57152.60951 & 15.5106 & 0.0093 &  $z$\\
3C323.1 & 57169.58816 & 15.4758 & 0.0094 &  $z$\\
3C323.1 & 57185.73522 & 15.4734 & 0.0062 &  $z$\\
3C323.1 & 57229.54058 & 15.4467 & 0.0047 &  $z$\\
3C323.1 & 57293.46063 & 15.4685 & 0.0167 &  $z$\\
3C323.1 & 57390.82173 & 15.3951 & 0.0056 &  $z$\\
3C323.1 & 57402.80516 & 15.4136 & 0.0043 &  $z$\\
3C323.1 & 57407.86596 & 15.4180 & 0.0058 &  $z$\\
3C323.1 & 57420.77584 & 15.4094 & 0.0045 &  $z$\\
3C323.1 & 57433.72091 & 15.4054 & 0.0049 &  $z$\\
3C323.1 & 57445.75992 & 15.4171 & 0.0105 &  $z$\\
4C09.72 & 57229.58331 & 15.9757 & 0.0096 &  $u$\\
4C09.72 & 57276.65023 & 16.1523 & 0.0064 &  $u$\\
4C09.72 & 57302.46231 & 16.2857 & 0.0079 &  $u$\\
4C09.72 & 57330.44826 & 16.2751 & 0.0073 &  $u$\\
4C09.72 & 57346.52437 & 16.3121 & 0.0158 &  $u$\\
4C09.72 & 57391.39393 & 16.3663 & 0.0117 &  $u$\\
4C09.72 & 57403.39828 & 16.3788 & 0.0111 &  $u$\\
4C09.72 & 57421.40847 & 16.4288 & 0.0179 &  $u$\\
4C09.72 & 57229.56485 & 15.7741 & 0.0047 &  $g$\\
4C09.72 & 57276.56819 & 15.9044 & 0.0028 &  $g$\\
4C09.72 & 57293.46705 & 16.0142 & 0.0396 &  $g$\\
4C09.72 & 57302.44352 & 15.9959 & 0.0034 &  $g$\\
4C09.72 & 57330.41384 & 16.0303 & 0.0028 &  $g$\\
4C09.72 & 57346.50540 & 16.0643 & 0.0131 &  $g$\\
4C09.72 & 57390.47603 & 16.1306 & 0.0046 &  $g$\\
4C09.72 & 57391.37494 & 16.1411 & 0.0070 &  $g$\\
4C09.72 & 57403.38318 & 16.1350 & 0.0053 &  $g$\\
4C09.72 & 57420.41671 & 16.1889 & 0.0055 &  $g$\\
4C09.72 & 57421.39121 & 16.1848 & 0.0064 &  $g$\\
4C09.72 & 57229.57618 & 15.9030 & 0.0040 &  $r$\\
4C09.72 & 57276.58061 & 16.0414 & 0.0032 &  $r$\\
4C09.72 & 57302.45512 & 16.1116 & 0.0038 &  $r$\\
4C09.72 & 57330.44056 & 16.1459 & 0.0033 &  $r$\\
4C09.72 & 57346.51708 & 16.1782 & 0.0135 &  $r$\\
4C09.72 & 57391.38666 & 16.2420 & 0.0054 &  $r$\\
4C09.72 & 57403.38501 & 16.2470 & 0.0042 &  $r$\\
4C09.72 & 57421.39744 & 16.2811 & 0.0057 &  $r$\\
4C09.72 & 57229.57050 & 15.8478 & 0.0052 &  $i$\\
4C09.72 & 57276.57442 & 15.9484 & 0.0042 &  $i$\\
4C09.72 & 57302.44931 & 16.0221 & 0.0048 &  $i$\\
4C09.72 & 57330.43425 & 16.0263 & 0.0055 &  $i$\\
4C09.72 & 57346.51123 & 16.0929 & 0.0247 &  $i$\\
4C09.72 & 57390.48183 & 16.1000 & 0.0064 &  $i$\\
4C09.72 & 57391.38074 & 16.1077 & 0.0071 &  $i$\\
4C09.72 & 57403.39033 & 16.1453 & 0.0081 &  $i$\\
4C09.72 & 57421.39160 & 16.1399 & 0.0083 &  $i$\\
4C09.72 & 57229.59182 & 15.7185 & 0.0061 &  $z$\\
4C09.72 & 57276.65914 & 15.7556 & 0.0048 &  $z$\\
4C09.72 & 57302.47097 & 15.7775 & 0.0056 &  $z$\\
4C09.72 & 57330.45773 & 15.8083 & 0.0051 &  $z$\\
4C09.72 & 57346.53310 & 15.7300 & 0.0098 &  $z$\\
4C09.72 & 57391.40255 & 15.8618 & 0.0073 &  $z$\\
4C09.72 & 57403.41184 & 15.8791 & 0.0063 &  $z$\\
4C09.72 & 57421.41588 & 15.8442 & 0.0151 &  $z$\\ [2pt]  
\hline\noalign{\vskip3pt} 
\end{tabular}}\label{lightucrve_table}
\begin{tabnote}
\hangindent6pt\noindent
\hbox to6pt{\footnotemark[$*$]\hss}\unskip% 
 The reported magnitude values are in AB magnitude system, and not corrected for Galactic extinction. A machine-readable version of the full table is available online.
\end{tabnote}
\end{table}


